Backward Reachability Analysis of Neural Feedback Loops: Techniques for Linear and Nonlinear Systems

As neural networks (NNs) become more prevalent in safety-critical applications such as control of vehicles, there is a growing need to certify that systems with NN components are safe. This paper presents a set of backward reachability approaches for safety certification of neural feedback loops (NFLs), i.e., closed-loop systems with NN control policies. While backward reachability strategies have been developed for systems without NN components, the nonlinearities in NN activation functions and general noninvertibility of NN weight matrices make backward reachability for NFLs a challenging problem. To avoid the difficulties associated with propagating sets backward through NNs, we introduce a framework that leverages standard forward NN analysis tools to efficiently find over-approximations to backprojection (BP) sets, i.e., sets of states for which an NN policy will lead a system to a given target set. We present frameworks for calculating BP over approximations for both linear and nonlinear systems with control policies represented by feedforward NNs and propose computationally efficient strategies. We use numerical results from a variety of models to showcase the proposed algorithms, including a demonstration of safety certification for a 6D system.

==> extra/_approach.tex <==
%!TEX root=main.tex

\section{Approach}
How do we do it???
\begin{itemize}
    \item General idea (single step)
    \item Iterative algorithm
    \item N-step refinement
    \item Hybrid (iterative+N-step) idk if we include this
    \item Nonlinear systems
    \item Partitioning Strategies
\end{itemize}
\iffalse
This section first outlines a technique to find one-step BP set over-approximations (\cref{alg:one_step_backprojection}) by solving a series of LPs. 
We then introduce \basic{}, which iteratively calls \cref{alg:one_step_backprojection} to calculate BP set estimates over a desired time horizon.
Finally, we propose \nstep{}, which further refines the BP set estimates from \basic{} with another series of LPs, thus reducing conservativeness with some additional computational cost.
% The tradeoffs between \basic{} and \nstep{} must therefore be considered when deciding which algorithms to use. 


\subsection{Over-Approximation of 1-Step Backprojection Sets} 
\label{sec:overapprox_one_step_BP}

% We first provide a summary of the proposed approach:
% \begin{enumerate}
%     \item Ignoring the NN, find (hyper-)rectangular bounds on the backreachable set (this is a superset of the BP set associated with the particular NN controller)
%     \item Within this region, relax the NN controller to acquire upper/lower affine bounds on control
%     \item Solve 2 LPs for each element of the state vector to compute states that will lead to the target set for some control effort within the upper/lower bounds
% \end{enumerate}
The proposed approach is as follows:
\begin{enumerate}
    \item Ignoring the NN and using control limits $\mathcal{U}$, solve two LPs for each element of the state vector to find the hyper-rectangular bounds $\bar{\mathcal{R}}_{-1}$ on the backreachable set $\mathcal{R}_{-1}$ (note that $\bar{\mathcal{R}}_{-1} \supseteq \mathcal{P}_{-1}$)
    \item Find upper/lower affine control bounds $\pi^U(\x_t)$ and $\pi^L(\x_t)$ by relaxing the NN controller (we use CROWN \cite{zhang2018efficient}, but other tools, e.g., \cite{weng2018towards, xu2020automatic}, could also be used) within the backreachable set
    \label{enum:nn_relaxation}
    \item Solve two LPs for each element of the state vector to compute hyper-rectangular bounds $\bar{\mathcal{P}}_{-1}$ on the states that will lead to the target set for \textit{some} control effort within the upper/lower bounds calculated in Step \ref{enum:nn_relaxation}
\end{enumerate}
The last step gives an over-approximation of the BP set, which is the set of interest.

The following lemma provides hyper-rectangle bounds on $\bar{\mathcal{P}}_{t}(\mathcal{X}_T)$ for a single timestep, which is the key component of the recursive algorithm introduced in the next section.

\begin{lemma}\label[lemma]{thm:backprojection}

Given an $m$-layer NN control policy $\pi:\R^{n_y}\to\R^{n_u}$, closed-loop dynamics $f: \R^{n_x} \times \Pi \to \R^{n_x}$ as in~\cref{eqn:ltv_dynamics,eqn:closed_loop_dynamics}, and target set $\mathcal{X}_T$, the set 
\begin{equation}
    \bar{\mathcal{P}}_{-1}(\mathcal{X}_T) = \{\x_t\ |\ \ubar{\x}_t \leq \x_t \leq \bar{\x}_t \}
\end{equation}
is a superset of the true BP set $\mathcal{P}_{-1}(\mathcal{X}_T)$,
where $\ubar{\mathbf{x}}_t$ and $\bar{\mathbf{x}}_t$ are computed elementwise by solving the LPs in~\cref{eqn:backprojection:lp_obj}.

\begin{proof}
Given dynamics~\cref{eqn:ltv_dynamics,eqn:closed_loop_dynamics} and constraints %$\mathcal{F_{\bar{R}}}$
% \begin{align}
% \bar{\bar{\mathbf{x}}}_{t; \istate} = \max_{\mathbf{x}_t, \mathbf{u}_t} \quad & \mathbf{x}_{t; \istate} \label{eqn:backreachable:lpmax_obj} \\
% \mathrm{s.t.} \quad & \mathbf{A} \mathbf{x}_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} \in \mathcal{X}_T \nonumber\\% \label{eqn:backreachable:lpmax_constr_state} \\
% & \mathbf{u}_t \in \mathcal{U} \nonumber\\% \label{eqn:backreachable:lpmax_constr_control} \\
% \ubar{\ubar{\mathbf{x}}}_{t; \istate} = \min_{\mathbf{x}_t, \mathbf{u}_t} \quad & \mathbf{x}_{t; \istate}  \label{eqn:backreachable:lpmin_obj} \\
% \mathrm{s.t.} \quad & \mathbf{A} \mathbf{x}_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} \in \mathcal{X}_T \nonumber\\% \label{eqn:backreachable:lpmin_constr_state} \\
% & \mathbf{u}_t \in \mathcal{U}, \nonumber% \label{eqn:backreachable:lpmin_constr_control}
% \end{align}
% Then, define the set of state and control constraints $\mathcal{F_P}$ as ,
\begin{equation}
\mathcal{F_{\bar{R}}} \triangleq \left\{
\mathbf{x}_t, \mathbf{u}_t\ \left| \
\begin{aligned}
& \mathbf{A} \mathbf{x}_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} \in \mathcal{X}_T,\\% \label{eqn:backreachable:lpmin_constr_state} \\
& \mathbf{u}_t \in \mathcal{U},
\end{aligned}\right.\kern-\nulldelimiterspace
\right\},
\label{eqn:backreachable:lp_constr}
\end{equation}
solve these optimization problems for each state $\istate \in [n_x]$,
\begin{equation}
\bar{\bar{\mathbf{x}}}_{t; \istate} = \min_{\mathbf{x}_t, \mathbf{u}_t \in \mathcal{F_{\bar{R}}}} \mathbf{e}_k^\top  \mathbf{x}_{t}, \quad \quad \ubar{\ubar{\mathbf{x}}}_{t; \istate} = \max_{\mathbf{x}_t, \mathbf{u}_t \in \mathcal{F_{\bar{R}}}} \mathbf{e}_k^\top  \mathbf{x}_{t}, \label{eqn:backreachable:lp_obj}
\end{equation}
where the notation $\mathbf{x}_{t;k}$ denotes the $k^\mathrm{th}$ element of $\mathbf{x}_t$ and $\mathbf{e}_k \ \in \R^{n_x}$ denotes the indicator vector, i.e., the vector with $k^\mathrm{th}$ equal to one and all other elements equal to zero. Eq. \cref{eqn:backreachable:lp_obj} provides a hyper-rectangular outer bound $\bar{\mathcal{R}}_{-1}(\mathcal{X}_T) \triangleq \{\mathbf{x}\ | \ \ubar{\ubar{\mathbf{x}}}_{t} \leq \mathbf{x}_{t} \leq \bar{\bar{\mathbf{x}}}_{t}\}$ on the backreachable set.
Note that this is a LP for the convex $\mathcal{X}_T,\ \mathcal{U}$ used here.

Given the bound, $\ubar{\ubar{\mathbf{x}}}_{t} \leq \mathbf{x}_{t} \leq \bar{\bar{\mathbf{x}}}_{t}$, \cref{thm:crown_particular_x} provides $\CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl$.
% which lead to the following inequalities based on~\cref{thm:particular_xt} with $\Aout=\mathbf{I}_{n_x}$, $\forall \istate \in [n_x]$,
% \begin{align}
% \begin{split}
% & \left[ \mathbf{A} \mathbf{x}_t + \mathbf{B} ( \Jbar{\mathbf{B}_{t; \istate, :}}{\CROWNAl}{\CROWNAu} \mathbf{y}_t + \Jbar{\mathbf{B}_{t; \istate, :}}{\CROWNbl}{\CROWNbu}) + \mathbf{c} \right]_{\istate} \\
%  \leq\ 
% & \mathbf{x}_{t+1; \istate} \\
%  \leq\ 
% & \left[ \mathbf{A} \mathbf{x}_t + \mathbf{B} ( \Jbar{\mathbf{B}_{t; \istate, :}}{\CROWNAu}{\CROWNAl} \mathbf{y}_t + \Jbar{\mathbf{B}_{t; \istate, :}}{\CROWNbu}{\CROWNbl}) + \mathbf{c} \right]_{\istate}.
% \end{split}
% \end{align}
Then, define the set of state and control constraints $\mathcal{F_{\bar{P}}}$ as
% \begin{align}
% \bar{\mathbf{x}}_{t; \istate} = \max_{\mathbf{x}_t, \mathbf{u}_t} \quad & \mathbf{x}_{t; \istate} \label{eqn:backprojection:lpmax_obj} \\
% \mathrm{s.t.} \quad & \mathbf{A} \mathbf{x}_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} \in \mathcal{X}_T \nonumber\\% \label{eqn:backprojection:lpmax_constr_state} \\
% & \mathbf{y}_t = \mathbf{C}\mathbf{x}_t \nonumber\\% \label{eqn:backprojection:lpmax_constr_output} \\
% & \pi^L(\y_t) \leq \mathbf{u}_t \leq \pi^U(\y_t) \nonumber\\% \label{eqn:backprojection:lpmax_constr_control} \\
% & \x_t \in \bar{\mathcal{R}}_{-1} \nonumber\\% \label{eqn:backprojection:lpmax_constr_backreach} \\
% \ubar{\mathbf{x}}_{t; \istate} = \min_{\mathbf{x}_t, \mathbf{u}_t} \quad & \mathbf{x}_{t; \istate} \label{eqn:backprojection:lpmin_obj} \\
% \mathrm{s.t.} \quad & \mathbf{A} \mathbf{x}_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} \in \mathcal{X}_T \nonumber\\% \label{eqn:backprojection:lpmin_constr_state} \\
% & \mathbf{y}_t = \mathbf{C}\mathbf{x}_t \nonumber\\% \label{eqn:backprojection:lpmin_constr_output} \\
% & \pi^L(\y_t) \leq \mathbf{u}_t \leq \pi^U(\y_t) \nonumber\\% \label{eqn:backprojection:lpmin_constr_control} \\
% & \x_t \in \bar{\mathcal{R}}_{-1} \nonumber% \label{eqn:backprojection:lpmin_constr_backreach},
% \end{align}
\begin{equation}
\mathcal{F_{\bar{P}}} \triangleq \left\{
\mathbf{x}_t, \mathbf{u}_t\ \left| \
\begin{aligned}
& \mathbf{A} \mathbf{x}_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} \in \mathcal{X}_T,\\% \label{eqn:backprojection:lpmax_constr_state} \\
& \pi^L(\x_t) \leq \mathbf{u}_t \leq \pi^U(\x_t), \\% \label{eqn:backprojection:lpmax_constr_control} \\
& \x_t \in \bar{\mathcal{R}}_{-1},% \label{eqn:backprojection:lpmax_constr_backreach} \\   
\end{aligned}\right.\kern-\nulldelimiterspace
\right\}
\label{eqn:backprojection:lp_constr}
\end{equation}
and solve the following optimization problems for each state $\istate \in [n_x]$:
\begin{equation}
\bar{\mathbf{x}}_{t; \istate} = \min_{\mathbf{x}_t, \mathbf{u}_t \in \mathcal{F_{\bar{P}}}} \mathbf{e}_k^\top \mathbf{x}_{t}, \quad \quad \ubar{\mathbf{x}}_{t; \istate} = \max_{\mathbf{x}_t, \mathbf{u}_t \in \mathcal{F_{\bar{P}}}} \mathbf{e}_k^\top \mathbf{x}_{t}. \label{eqn:backprojection:lp_obj}
\end{equation}

% After substituting in for $\mathbf{y}_t$, grouping $\mathbf{x}_t$ terms together, and using \cref{eqn:backreachable:zba,eqn:backreachable:zbb,eqn:backreachable:zbc,eqn:backreachable:zbd},
% \begin{align}
% \begin{split}
% & \left(\mathbf{A} + \mathbf{Z}^{\mathbf{B}\CROWNAl\CROWNAu}\right) \mathbf{x}_{t} + \mathbf{z}^{\mathbf{B}\CROWNbl\CROWNbu} + \mathbf{c} \\
%  \leq\ 
% & \mathbf{x}_{t+1} \\
%  \leq\ 
% & \left(\mathbf{A} + \mathbf{Z}^{\mathbf{B}\CROWNAu\CROWNAl}\right) \mathbf{x}_{t} + \mathbf{z}^{\mathbf{B}\CROWNbu\CROWNbl} + \mathbf{c}
% \label{eqn:backproj:relaxed_nn_bounds}.
% \end{split}
% \end{align}
% \cref{eqn:backprojection:lpmax_obj,eqn:backprojection:lpmax_constr_state,eqn:backprojection:lpmax_constr_output,eqn:backprojection:lpmax_constr_control,eqn:backprojection:lpmax_constr_backreach,eqn:backprojection:lpmin_obj,eqn:backprojection:lpmin_constr_state,eqn:backprojection:lpmin_constr_output,eqn:backprojection:lpmin_constr_control,eqn:backprojection:lpmin_constr_backreach}

The LPs solved in  \cref{eqn:backprojection:lp_obj} provide a hyper-rectangular outer bound of the BP set, i.e.,
\begin{align}
    \bar{\mathcal{P}}_{-1}(\mathcal{X}_T) = &\ \{\x_t\ |\ \ubar{\x}_t \leq \x_t \leq \bar{\x}_t \}
    \label{eqn:BPproof:rect_bound} \\ 
    \begin{split}
         \supseteq & \ \{\x_t\ |\ \mathbf{A} \x_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} \in \mathcal{X}_T,\ \\ & \quad \quad \quad \quad \pi^L(\x_t) \leq \mathbf{u}_t \leq \pi^U(\x_t)\},
    \end{split} \label{eqn:BPproof:true_relaxed_BP} \\
    \supseteq &\ \mathcal{P}_{-1}(\mathcal{X}_T).
    \label{eqn:BPproof:true_BP}
\end{align}
$\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ is the hyper-rectangular outer bound of \cref{eqn:BPproof:true_relaxed_BP}, thus guaranteeing the relationship between \cref{eqn:BPproof:rect_bound} and \cref{eqn:BPproof:true_relaxed_BP}.
The relation between \cref{eqn:BPproof:true_relaxed_BP} and \cref{eqn:BPproof:true_BP} holds because $\pi^L(\x_t) \leq \pi(\x_t) \leq \pi^U(\x_t)$ (via \cref{thm:crown_particular_x}). 
It follows that $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T) \supseteq \mathcal{P}_{-1}(\mathcal{X}_T)$.
%Denote $\ubar{\mathbf{x}}_t$ and $\bar{\mathbf{x}}_t$ as the minimum and maximum values of $\mathbf{x}_t$ for which there exists some $\mathbf{u}_t \in [\pi^L(\y_t),\ \pi^U(\y_t)]$ and which lead to $\x_{t+1} \in \mathcal{X}_T$. Defining $\bar{\mathcal{P}}_{-1} = \{\x_t\ |\ \ubar{\x}_t \leq \x_t \leq \bar{\x}_t\}$, it follows that the backprojection set $\mathcal{P}_{-1}$ = \{$\x_t\ |\ \mathbf{A} \x_t+ \mathbf{B} \pi(\y_t) \in \mathcal{X}_T\} $ for which  is a subset of the (hyper-)rectangle bounded by $\ubar{\x}_t$ and $\bar{\x}_t$.
\end{proof}
\end{lemma}

Note that we relaxed the NN over the entire range of $\bar{\mathcal{R}}_{-1}$, but if we instead divide it into smaller regions and relax each of them individually, we may find tighter bounds on the control input.
While partitioning $\bar{\mathcal{R}}_{-1}$ in this way is not required, it can be used to reduce the conservativeness of the BP estimate at the cost of increased computation time associated with solving LPs for each partitioned region.
Ref.~\cite{everett2021reachability} provides a detailed discussion on different partitioning strategies.

% \begin{corollary}
% The set $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ composed of all $\mathbf{x}_t$ that satisfy~\cref{eqn:backreachable:polytope} is a superset of the one-step backprojection set, $\mathcal{P}_{-1}(\mathcal{X}_T)$.

% \begin{proof}
% Suppose $\mathbf{x}_t$ satisfies \cref{eqn:backreachable:polytope}, i.e., $\mathbf{x}_t \in \bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$.
% \mfe{TODO: Finish this}
% \nr{may have misunderstood what you intended to do with lem IV.1, but this was done there}

% Thus, $\mathbf{x}_t$ also satisfies the inequalities~\cref{eqn:backproj:lower_next_state,eqn:backproj:upper_next_state}, and thus also \cref{eqn:backproj:relaxed_nn_bounds}.
% Since $\mathbf{x}_{t+1}=f(\mathbf{x}_t; \pi)$, $\mathbf{x}_t$ also satisfies $\ubar{\mathbf{x}}_{t+1} \leq f(\mathbf{x}_t; \pi) \leq \bar{\mathbf{x}}_{t+1}$, which means that $\mathbf{x}_t \in \mathcal{P}_{-1}(\mathcal{X}_T)$ as well.
% Thus, $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T) \subseteq \mathcal{P}_{-1}(\mathcal{X}_T)$.
% \end{proof}
% \end{corollary}


\subsection{Algorithm for Computing Backprojection Sets}

\begin{algorithm}[t]
 \caption{oneStepBackproj}
 \begin{algorithmic}[1]
 \setcounter{ALC@unique}{0}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE target state set $\mathcal{X}_T$, trained NN control policy $\pi$, partition parameter $\mathbf{r}$
 \ENSURE BP set approximations $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$,
 affine control bound parameters
 $\mathbf{\Omega}_{-1}$
    \STATE $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T) \leftarrow \emptyset$
    \STATE $\bar{\mathcal{R}}_{t}(\mathcal{X}_T)\! =\! [\ubar{\ubar{\mathbf{x}}}_{t}, \bar{\bar{\mathbf{x}}}_{t}]\! \leftarrow\! \mathrm{backreach}(\bar{\mathcal{P}}_{t\text{+}1}(\mathcal{X}_T), \mathcal{U})$ % \textbackslash  \textbackslash  Eq.\! \cref{eqn:backreachable:lp_obj} \label{alg:one_step_backprojection:backreach} \\
    \STATE $\mathcal{S} \leftarrow \mathrm{partition}([\ubar{\ubar{\mathbf{x}}}_{t}, \bar{\bar{\mathbf{x}}}_{t}], \mathbf{r})$
    \FOR{$[\ubar{\mathbf{x}}_{t}, \bar{\mathbf{x}}_{t}]$ in $\mathcal{S}$}
        \STATE $\CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl \leftarrow \mathrm{CROWN}(\pi, [\ubar{\mathbf{x}}_{t}, \bar{\mathbf{x}}_{t}])$ % \textbackslash \textbackslash \ Eq. \cref{eq:f_j_UL} 
        \FOR{$\istate \in n_x$}
            \STATE $\bar{\bar{\mathbf{x}}}_{t;k} \leftarrow \mathrm{lpMax}(\mathcal{X}_T,\bar{\mathcal{R}}_t, \CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl)$ % \!  \textbackslash \textbackslash \ Eq. \cref{eqn:backprojection:lp_obj} 
            \STATE $\ubar{\ubar{\mathbf{x}}}_{t;k} \leftarrow \mathrm{lpMin}(\mathcal{X}_T,\bar{\mathcal{R}}_t,\CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl)$ % \ \textbackslash \textbackslash \ Eq. \cref{eqn:backprojection:lp_obj}
        \ENDFOR
        \STATE $\mathcal{A} \leftarrow \{\mathbf{x}\ \lvert\ \forall \istate \in n_x,\ \ubar{\ubar{\mathbf{x}}}_{t;k} \leq \mathbf{x} \leq \bar{\bar{\mathbf{x}}}_{t;k}\}$
        \STATE $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T) \leftarrow \bar{\mathcal{P}}_{-1}(\mathcal{X}_T) \cup \mathcal{A}$ \label{alg:one_step_backprojection:union}
    \ENDFOR
    % \STATE $\bar{\bar{\mathbf{x}}}_{t} \leftarrow \mathrm{max}(\{\mathbf{x}\ \lvert\ \forall \istate \in n_x,\ x_k \in \bar{\mathcal{P}}_{-1}(\mathcal{X}_T)\})$
    % \STATE $\ubar{\ubar{\mathbf{x}}}_{t}, \ubar{\ubar{\mathbf{x}}}_{t;k} \leftarrow \mathrm{min}(\{\mathbf{x}\ \lvert\ \forall \istate \in n_x,\ x_k \in \bar{\mathcal{P}}_{-1}(\mathcal{X}_T)\})$
    \STATE $[\bar{\bar{\mathbf{x}}}'_{t},\ \ubar{\ubar{\mathbf{x}}}'_{t}] \leftarrow \text{boundWithRectangle}(\bar{\mathcal{P}}_{-1}(\mathcal{X}_T))$
    \STATE $\mathbf{\Omega}_{-1} = [\bar{\CROWNAu}, \bar{\CROWNAl}, \bar{\CROWNbu}, \bar{\CROWNbl}] \leftarrow \mathrm{CROWN}(\pi, [\ubar{\ubar{\mathbf{x}}}'_{t}, \bar{\bar{\mathbf{x}}}'_{t}])$
 \RETURN $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T),\ \mathbf{\Omega}_{-1}$ \label{alg:one_step_backprojection:return}
 \end{algorithmic}\label{alg:one_step_backprojection}
\end{algorithm}

\cref{alg:one_step_backprojection} follows the procedure outlined in \cref{sec:overapprox_one_step_BP} and \cref{thm:backprojection} to obtain $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$, i.e., an over-approximation of the BP set for a single timestep.
The functions {\tt lpMax} and {\tt lpMin} solve the LPs formulated by \cref{eqn:backprojection:lp_obj} and {\tt backreach} solves the LPs formulated by \cref{eqn:backreachable:lp_obj}.
The partition parameter $\mathbf{r} \in \mathds{R}^{n_x}$ gives the option to uniformly split the backreachable set, e.g., $\mathbf{r} = [2,3]$ will split $\bar{\mathcal{R}}_{-1}(\mathcal{X}_T)$ into a $2 \times 3$ grid of cells.

To provide safety guarantees over an extended time horizon $\tau$, we extend this idea to iteratively compute BPs at multiple timesteps $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T)$. 
We first initialize the zeroth BP set as the target set (\cref{alg:backprojection:initialize}). 
Then we step backward in time (\cref{alg:backprojection:timestep_for_loop}), recursively using \cref{alg:one_step_backprojection} ({\tt oneStepBackproj}), and the BP from the previous step to iteratively compute the new BP set (\cref{alg:backprojection:one_step_backproj_iter}). 
This is done $\tau$ times to give a list of BP set estimates $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T)$.
The proposed procedure is summarized in \cref{alg:backprojection}.



\begin{algorithm}[t]
 \caption{\basic}
 \begin{algorithmic}[1]
 \setcounter{ALC@unique}{0}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE target state set $\mathcal{X}_T$, trained NN control policy $\pi$, time horizon $\tau$, partition parameter $\mathbf{r}$
 \ENSURE BP set approximations $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T)$,
 affine control bound parameters
 $\mathbf{\Omega}_{-\tau:-1}$
    \STATE $\bar{\mathcal{P}}_{0}(\mathcal{X}_T) \leftarrow \mathcal{X}_T$ \label{alg:backprojection:initialize}
    \FOR{$t$ in $\{-1, -2, \ldots, -\tau\}$} \label{alg:backprojection:timestep_for_loop}
        \STATE $\bar{\bar{\mathcal{P}}}_{t+1}(\mathcal{X}_T) \leftarrow \text{boundWithRectangle}(\bar{\mathcal{P}}_{t+1}(\mathcal{X}_T))$ \label{alg:backprojection:bound_with_rect}
        \STATE $\bar{\mathcal{P}}_{t}(\mathcal{X}_T), \mathbf{\Omega}_t \leftarrow \text{oneStepBackproj}(\bar{\bar{\mathcal{P}}}_{t+1}(\mathcal{X}_T), \pi, \mathbf{r})$ \label{alg:backprojection:one_step_backproj_iter}
    \ENDFOR
 \RETURN $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T),\ \mathbf{\Omega}_{-\tau:-1}$ \label{alg:backprojection:return}
 \end{algorithmic}\label{alg:backprojection}
\end{algorithm}

\subsection{Algorithm for Computing N-Step Backprojection Sets}
Notice that by iteratively making over-approximations using the previously calculated BP over-approximation, \basic{} tends to accrue conservativeness over the time horizon due to the wrapping effect \cite{le2009reachability}.
Thus even if $\bar{\mathcal{P}}_{-\tau}(\mathcal{X}_T)$ tightly bounds the set of states that reach $\bar{\mathcal{P}}_{-\tau+1}(\mathcal{X}_T)$, it may be an overly conservative estimate of the set of states that ultimately end up in $\mathcal{X}_T$ in $\tau$ timesteps.
To reduce the accrued conservativeness, we present \nstep{} (\cref{alg:Nbackprojection}) that uses \basic{} to initialize $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T)$ and the collected affine control bound parameters $\mathbf{\Omega}_{-\tau:-1}$. 
We then use a procedure similar to the one outlined in \cref{sec:overapprox_one_step_BP}, but now we relax the NN over $\bar{\mathcal{P}}_t$ instead of $\bar{\mathcal{R}}_t$ and include additional constraints that require the future states of the system to progress through the future BP estimates and eventually reach the target set while satisfying the relaxed affine control bounds at each step along the way.

\begin{lemma}\label[lemma]{thm:Nbackprojection}

Given an $m$-layer NN control policy $\pi:\R^{n_x}\to\R^{n_u}$, closed-loop dynamics $f: \R^{n_x} \times \Pi \to \R^{n_x}$ as in~\cref{eqn:ltv_dynamics,eqn:closed_loop_dynamics}, a set of BP estimates $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T)$, a corresponding set of affine control bounds $\mathbf{\Omega}_{-\tau:-1}$, and target set $\mathcal{X}_T$, the following relations hold:
\begin{equation*}
    \mathcal{P}_{t}(\mathcal{X}_T) \subseteq \bar{\mathcal{P}}'_t(\mathcal{X}_T) \subseteq \bar{\mathcal{P}}_t(\mathcal{X}_T), \forall t \in \underbrace{\{\text{-}\tau, \text{-}\tau+1, \ldots, -1\}}_{\triangleq \mathcal{T}},
\end{equation*}
where $\bar{\mathcal{P}}'_t(\mathcal{X}_T) \triangleq \{\x_{t}\ |\ \ubar{\mathbf{x}}'_{t} \leq \mathbf{x}_{t} \leq \bar{\mathbf{x}}'_{t} \}$ with $\ubar{\mathbf{x}}'_{t}$ and $\bar{\mathbf{x}}'_{t}$ calculated using the LPs specified by \cref{eqn:Nbackprojection:lp_obj}.

\begin{proof}
Given dynamics from~\cref{eqn:ltv_dynamics,eqn:closed_loop_dynamics}, solve the following optimization problems for each state $\istate \in [n_x]$ and for each $t \in \mathcal{T}$,
\begin{equation}
\bar{\mathbf{x}}_{t; \istate} = \min_{\mathbf{x}_t, \mathbf{u}_t \in \mathcal{F}_{\bar{\mathcal{P}}'_t}} \mathbf{e}_k^\top \mathbf{x}_{t}, \quad \quad \ubar{\mathbf{x}}_{t; \istate} = \max_{\mathbf{x}_t, \mathbf{u}_t \in \mathcal{F}_{\bar{\mathcal{P}}'_t}} \mathbf{e}_k^\top \mathbf{x}_{t}, \label{eqn:Nbackprojection:lp_obj}
\end{equation}
where
% \begin{align}
% \bar{\mathbf{x}}'_{t; \istate} = \max_{\mathbf{x}_t, \mathbf{u}_t} \quad & \mathbf{x}_{t; \istate} \label{eqn:Nbackprojection:lpmax_obj} \\
% \mathrm{s.t.} \quad & \nonumber \\
% \!\!\!\!\!\!\forall \mathfrak{t} \in \mathfrak{T} &
% \begin{cases} \notag
% \mathbf{A} \mathbf{x}_{\mathfrak{t}} + \mathbf{B} \mathbf{u}_{\mathfrak{t}} + \mathbf{c} 
% %\\ \qquad \qquad \qquad \qquad 
% \in \bar{\mathcal{P}}_{\mathfrak{t}+1}, \\
% \mathbf{y}_{\mathfrak{t}} = \mathbf{C}\mathbf{x}_{\mathfrak{t}}, \\
% \pi^L_\mathfrak{t}(\y_{\mathfrak{t}}) \leq \mathbf{u}_{\mathfrak{t}} \leq \pi^U_\mathfrak{t}(\y_{\mathfrak{t}}), \\
% \x_\mathfrak{t} \in \bar{\mathcal{P}}_\mathfrak{t}(\mathcal{X}_T),
% \end{cases}\\
% \ubar{\mathbf{x}}'_{t; \istate} = \min_{\mathbf{x}_t, \mathbf{u}_t} \quad & \mathbf{x}_{t; \istate} \label{eqn:Nbackprojection:lpmin_obj} \\
% \mathrm{s.t.} \quad &  \nonumber \\ 
% \!\!\!\!\!\!\forall \mathfrak{t} \in \mathfrak{T} &
% \begin{cases} \notag
% \mathbf{A} \mathbf{x}_{\mathfrak{t}} + \mathbf{B} \mathbf{u}_{\mathfrak{t}} + \mathbf{c} 
% %\\ \qquad \qquad \qquad \qquad 
% \in \bar{\mathcal{P}}_{\mathfrak{t}+1}, \\
% \mathbf{y}_{\mathfrak{t}} = \mathbf{C}\mathbf{x}_{\mathfrak{t}}, \\
% \pi^L_\mathfrak{t}(\y_{\mathfrak{t}}) \leq \mathbf{u}_{\mathfrak{t}} \leq \pi^U_\mathfrak{t}(\y_{\mathfrak{t}}), \\
% \x_\mathfrak{t} \in \bar{\mathcal{P}}_\mathfrak{t}(\mathcal{X}_T),
% \end{cases}
% \end{align}
\begin{equation}
\mathcal{F}_{\bar{\mathcal{P}}'_t} \! \triangleq \! \left\{
\! \mathbf{x}_{t}, \mathbf{u}_{t} \left| \ 
\begin{aligned}
& \mathbf{A} \mathbf{x}_t + \mathbf{B} \mathbf{u}_t + \mathbf{c} = \x_{t+1}. \\
& \x_{t+1} \in \bar{\mathcal{P}}_{t+1}, \\% \label{eqn:backprojection:lpmax_constr_state} \\
& \pi^L_t(\x_{t}) \leq \mathbf{u}_{t} \leq \pi^U_t(\x_t),\\% \label{eqn:backprojection:lpmax_constr_control} \\
& \x_t \in \bar{\mathcal{P}}_t(\mathcal{X}_T), % \label{eqn:backprojection:lpmax_constr_backreach} \\   
\end{aligned}\right.\kern-\nulldelimiterspace 
% \quad \forall t \in \mathcal{T}
\right\},
\label{eqn:Nbackprojection:lp_constr}
\end{equation}
with $\bar{\mathcal{P}}_0(\mathcal{X}_T) = \mathcal{X}_T$, and $\pi^L_t$ and $\pi^U_t$ obtained from $\mathbf{\Omega}_{-\tau:-1}$.

The final constraint in \cref{eqn:Nbackprojection:lp_constr} guarantees $\bar{\mathcal{P}}'_t(\mathcal{X}_T) \subseteq \bar{\mathcal{P}}_t(\mathcal{X}), \forall t \in \mathcal{T}$.
The third constraint ensures that the relations \cref{eqn:BPproof:rect_bound,eqn:BPproof:true_relaxed_BP,eqn:BPproof:true_BP} in the proof of \cref{thm:backprojection} holds for all $t \in \mathcal{T}$, thus guaranteeing $\mathcal{P}_{t}(\mathcal{X}_T) \subseteq \bar{\mathcal{P}}'_t(\mathcal{X}_T)$. It follows that $\mathcal{P}_{t}(\mathcal{X}_T) \subseteq \bar{\mathcal{P}}'_t(\mathcal{X}_T) \subseteq \bar{\mathcal{P}}_t(\mathcal{X}), \forall t \in \mathcal{T}$.
\end{proof}
\end{lemma}

Notice that the first two constraints provide the key advantage of the LPs solved by \cref{eqn:Nbackprojection:lp_obj} over those given by \cref{thm:backprojection} in that they require the state to trace back through the set of BPs leading to the original target set, thus providing a better approximation of the true BP set. 





\begin{algorithm}[t]
 \caption{\nstep}
 \begin{algorithmic}[1]
 \setcounter{ALC@unique}{0}
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \renewcommand{\algorithmicensure}{\textbf{Output:}}
 \REQUIRE target state set $\mathcal{X}_T$, trained NN control policy $\pi$, time horizon $\tau$, partition parameter $\mathbf{r}$
 \ENSURE Refined BP set approximations $\bar{\mathcal{P}}'_{-\tau:0}(\mathcal{X}_T)$
    \STATE $\bar{\mathcal{P}}'_{-\tau:0}(\mathcal{X}_T) \leftarrow \emptyset$
    \STATE $\bar{\mathcal{P}}_{-\tau:0}(\mathcal{X}_T),\ \mathbf{\Omega}_{-\tau:-1} \leftarrow \! \text{\basic}(\mathcal{X}_T, \pi, \tau, \mathbf{r})$
    \STATE $\bar{\mathcal{P}}'_{-1:0}(\mathcal{X}_T) \leftarrow \bar{\mathcal{P}}_{-1:0}(\mathcal{X}_T)$
    \FOR{$t$ in $\{-2, \ldots, -\tau\}$} \label{alg:Nbackprojection:timestep_for_loop}
        \STATE $[\ubar{\ubar{\mathbf{x}}}_{t}, \bar{\bar{\mathbf{x}}}_{t}] \leftarrow \text{boundWithRectangle}(\bar{\mathcal{P}}_{t}(\mathcal{X}_T))$
        \STATE $\mathcal{S} \leftarrow \mathrm{partition}([\ubar{\ubar{\mathbf{x}}}_{t}, \bar{\bar{\mathbf{x}}}_{t}], \mathbf{r})$
        \FOR{$[\ubar{\mathbf{x}}_{t}, \bar{\mathbf{x}}_{t}]$ in $\mathcal{S}$}
            \STATE $\CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl \leftarrow \mathrm{CROWN}(\pi, [\ubar{\mathbf{x}}_{t}, \bar{\mathbf{x}}_{t}])$
            \FOR{$\istate \in n_x$}
                \STATE $\bar{\bar{\mathbf{x}}}_{t;k} \leftarrow \! \mathrm{NStepLpMax}(\bar{\mathcal{P}}_{\text{-}\tau:0}, \mathbf{\Omega}_{\text{-}\tau:\text{-}1},\CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl)$
                \STATE $\ubar{\ubar{\mathbf{x}}}_{t;k} \leftarrow \! \mathrm{NStepLpMin}(\bar{\mathcal{P}}_{\text{-}\tau:0},\ \mathbf{\Omega}_{\text{-}\tau:\text{-}1},\CROWNAu, \CROWNAl, \CROWNbu, \CROWNbl)$
            \ENDFOR
            \STATE $\mathcal{A} \leftarrow \{\mathbf{x}\ \lvert\ \forall \istate \in n_x,\ \ubar{\ubar{\mathbf{x}}}_{t;k} \leq \mathbf{x} \leq \bar{\bar{\mathbf{x}}}_{t;k}\}$
            \STATE $\bar{\mathcal{P}}'_{-1}(\mathcal{X}_T) \leftarrow \bar{\mathcal{P}}_{-1}(\mathcal{X}_T) \cup \mathcal{A}$ \label{alg:Nbackprojection:union}
        \ENDFOR
        \STATE $\bar{\mathcal{P}}'_t(\mathcal{X}_T) \leftarrow \bar{\mathcal{P}}'_{-1}(\mathcal{X}_T)$
    \ENDFOR
 \RETURN $\bar{\mathcal{P}}'_{-\tau:0}(\mathcal{X}_T)$ \label{alg:Nbackprojection:return}
 \end{algorithmic}\label{alg:Nbackprojection}
\end{algorithm}
\fi





==> extra/_intro.tex <==
%!TEX root=main.tex

\section{Introduction}
\begin{outline}
    \1 NNs in control
        \2 Applications
            \3 Autonomous driving \cite{chen2015deepdriving}
            \3 Collision avoidance \cite{julian2019deep}
        \2 Need for NN verification
    \1 NN analysis
        \2 Open-loop \cite{zhang2018efficient, weng2018towards, katz2017reluplex, bunel2018unified, tjeng2017evaluating, liu2019algorithms,  katz2019marabou, jia2021verifying, raghunathan2018semidefinite}
        \2 Closed-loop
            \3 Linear \cite{ivanov2019verisig}
                \4 Forward reachability \cite{dutta2019reachability, huang2019reachnn, fan2020reachnn, hu2020reach, xiang2020reachable, everett2021reachability}
                \4 Backward reachability \cite{vincent2021reachable, everett2021reachability, bak2022closed}
            \3 Nonlinear
                \4 Forward reachability \cite{sidrane2021overt}
    \1 Challenge
        \2 Classical Reachability \cite{bansal2017hamilton, evans1998partial, mitchell2007comparing}
            \3 Tools \cite{frehse2011spaceex, chen2013flow, althoff2015introduction, duggirala2015c2e2, bak2017hylaa, bogomolov2019juliareach}
        \2 Problems with NFLs in particular
    \1 Our work BReach? BRaNFul? BReNFeL? BaR-NFL? BReach-NFL? BaRreN?
        \2 Ideas hinge on \cite{sidrane2021overt, rober2022backward}
        \2 High level method outline
            \3 Do we just present full strategy (i.e. include nonlinear in general method outline)?
    \1 Contributions
        \2 Method to calculate backward reachable sets for nonlinear NFLs with general activation functions.
        \2 Partitioning strategy to reduce conservativeness
        \2 Demonstration of scalability and numerical results showing successful analysis of a 6th order system
            
        
    
            
            
\end{outline}

==> extra/_preliminaries.tex <==
%!TEX root=main.tex

\section{Preliminaries}
\begin{outline}
\1 System
\1 Nonlinear over-approximation
\1 NN weights + formulation
\1 NN verification
    \2 LP ball
    \2 Crown Bounds
    \3 Need to figure out how to mesh Stanford NN verification strategy
\1 Reachability notation and definitions
\end{outline}

\subsection{System dynamics}
We consider a discrete-time time-invariant nonlinear system with dynamics given by
\begin{equation}
    \mathbf{x}_{t+1} = f(\mathbf{x}_t, \mathbf{u}_t)
\end{equation}
where $\mathbf{x}_t \in \mathds{R}^{n_x}$, $\mathbf{u}_t \in \mathds{R}^{n_u}$.
The dynamics $f$ are assumed known and $\mathbf{u}_t$ is a state-feedback control policy specified by an $m$-layer feedforward NN  $\pi(\cdot)$, i.e., $\mathbf{u}_t = \pi(\mathbf{x}_t)$. We assume $\mathbf{u}_t$ is constrained by control limits and is thus limited to the convex set of legal control values $\mathcal{U}$, i.e., $\mathbf{u}_t \in \mathcal{U}$. Similarly, we consider $\mathbf{x}_t$ to be constrained to an operating region of the state space $\mathcal{X}$, i.e., $\mathbf{x}_t \in \mathcal{X}$.

\subsection{Linear Over-Approximation of Nonlinear Systems}

\subsection{Neural Network Policy}
A feedforward NN $\pi(\cdot)$ with $L$ hidden layers (and two additional layers for input and output) is considered.
The number of neurons in layer $l$ is denoted by $n^l\ \forall l \in [L+1]$ where $[i]$ denotes the set $\{0,1, ..., i\}$. 
For a given input $\mathbf{x} \in \mathds{R}^{n^0}$ to the NN, the output is formulated by the following series of calculations:
\begin{align}
\begin{split}
    \x^{0} &= \x \\
    \z^{l} &= \mathbf{W}^{l} \x^{l}+\mathbf{b}^{l}, \forall l\in[L] \\
    \x^{l+1} &= \sigma^{l}(\z^{l}), \forall l\in[L-1] \\
    \pi(\x) &= \z^{L},
\end{split}
\end{align}
where $\mathbf{W}^{l} \in \mathds{R}^{n^{l+1} \times n^{l}}$ and $\mathbf{b}^{l} \in \mathds{R}^{n^{l+1}}$ are the $l^\mathrm{th}$-layer weight matrix and bias vector, respectively, $\z^{l} \in \mathds{R}^{n^{l+1}}$ is the vector of pre-activation values, and $\x^{l+1} \in \mathds{R}^{n^{l+1}}$ is the layer's output, calculated by passing the pre-activation vector through an activation function $\sigma^l(\cdot): \R^{n_{l+1}} \to \R^{n_{l+1}}$ such as the ReLU, tanh, or other activation functions handled by CROWN \cite{zhang2018efficient} \nr{TODO: overt verification activation functions?}.

\subsection{Neural Network Verification}

\subsection{Backward Reachability Analysis}
The goal of backward reachability analysis is to determine the set of states that a control policy $\pi$ will drive to a given target set of states $\mathcal{X}_T$. 
In \cref{fig:backreachable} we introduce notation to define several sets of interest for backward reachability analysis of NFLs.
The one-step backreachable set $\mathcal{R}_{-1}(\mathcal{X}_T)$ defines the set of all states for which there exists some control value $\mathbf{u}_{-1} \in \mathcal{U}$ that will drive the system to $\mathcal{X}_T$.
The backprojection set $\mathcal{P}_{-1}(\mathcal{X}_T)$ is then defined as the set of states for which $\mathbf{u}_{-1}=\pi(\mathbf{x}_{-1})$ will drive the system to $\mathcal{X}_T$.
Notice that by clipping the output of $\pi$ as is done in \cite{hu2020reach}, we can guarantee that $\pi(\mathbf{x}_{-1}) \subseteq \mathcal{U}$, thus implying that  $\mathcal{P}_{-1} \subseteq \mathcal{R}_{-1}$. 



\begin{figure}[t]
\begin{tikzpicture}

    \draw [red, ultra thick] (2.5,-0.5) rectangle (4,0.5) node[above] {$\mathcal{X}_{T}$};
    
    \draw [fill=black!20!green!60!white]  plot[smooth, tension=.7] coordinates {(-3,2.5) (-3.5,2.2) (-4,1.8) (-3.5,0) (-3.5,-1.8) (-2.5,-1.9) (0,-1.7) (-0.3,0.1) (-1,1.5) (-2.3,2.5) (-3,2.5)} node[above] {$\mathcal{R}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a) at (-2.6,2.4) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b) at (3.55,0.2) {};
    \draw [->,blue, ultra thick] (a.east) to [out=5,in=75] (b.north);
    \node[black] (RTset) at (1.3,2.7) {$\exists \mathbf{u} \in \mathcal{U}$};

    \draw [fill=black!10!white]  plot[smooth, tension=.7] coordinates {(-2.9,1.6) (-1.5,1.3) (-0.2,-1.0) (-1.1,-1.8) (-3.2,-1.2) (-3,0.1) (-3.7,1.1) (-2.9,1.6)} node[above] {$\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c) at (-2.3,1.4) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d) at (2.8,0.2) {};
    \draw [->,blue, ultra thick] (c.east) to [out=350,in=120] (d.north);
    \node[black] (PTbarset) at (1, 1.65) {$\exists \mathbf{u} \in [\pi^L(\mathbf{x}_{-1}), \pi^U(\mathbf{x}_{-1})]$};

    \draw [fill=black!40!white]  plot[smooth, tension=.7] coordinates {(-2.1,0.7) (-1.5,0.45) (-0.5,-0.8) (-1.4,-1.6) (-2.8,-0.8) (-2.6,0.45) (-2.1,0.7)} node[above] {$\mathcal{P}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e) at (-2,0.35) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (f) at (3.0,-0.2) {};
    \draw [->,blue, ultra thick] (e.east) to [out=15,in=190] (f.west);
    \node[black] (PTset) at (1.2, -0.5) {$\mathbf{u} = \pi(\mathbf{x}_{-1})$};

    \draw [fill=black!20!white]  plot[smooth, tension=.7] coordinates {(-1.95,-0.4) (-1.4,-0.7) (-0.6,-0.8) (-1.1,-1.4) (-2.8,-0.8) (-1.95,-0.4)} node[above] {$\ubar{\mathcal{P}}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c) at (-1.0,-1.25) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d) at (3.8,-.4) {};
    \draw [->,blue, ultra thick] (c.east) to [out=360,in=240] (d.south);
    \node[black] (PTbarset) at (2.1, -1.8) {$\forall \mathbf{u} \in [\pi^L(\mathbf{x}_{-1}), \pi^U(\mathbf{x}_{-1})]$};

\end{tikzpicture}
\caption{
One-step backreachable set $\mathcal{R}_{-1}$ and backprojection set $\mathcal{P}_{-1}$ for a given target set $\mathcal{X}_T$. 
$\mathcal{R}_{-1}$ contains all states for which there exists a control that will drive the system to $\mathcal{X}_T$ in one timestep.
$\mathcal{P}_{-1}$ contains all states for which the NN controller will drive the system to $\mathcal{X}_T$ in one timestep.
BP under-approximation $\protect\ubar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ and over-approximation $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ define regions where \textit{all} and \textit{some}, respectively, of the relaxed NN controls will drive the system to $\mathcal{X}_T$.}
\label{fig:backreachable}
\vspace*{-0.12in}
\end{figure}


\iffalse
\subsection{System Dynamics}

We first assume that the system of interest can be described by the linear discrete-time system,
\begin{align}
\begin{split}
    \mathbf{x}_{t+1} & = \mathbf{A} \mathbf{x}_{t} + \mathbf{B} \mathbf{u}_t + \mathbf{c} \label{eqn:ltv_dynamics} \\
    \mathbf{y}_{t} & = \mathbf{C}^T\mathbf{x}_t,
\end{split}
\end{align}
where $\mathbf{x}_t\in\R^{n_x},\, \mathbf{u}_t\in\R^{n_u},\, \mathbf{y}_t\in\R^{n_y}$ are state, control, and output vectors, $\mathbf{A},\, \mathbf{B},\, \mathbf{C}$ are known system matrices, and $\mathbf{c}\in\R^{n_x}$ is a known exogenous input.
%
We assume the control input is constrained by control limits, i.e., $\mathbf{u}_t\in\mathcal{U}$, and is determined by a state-feedback control policy $\mathbf{u}_t=\pi(\mathbf{x}_t)$ (i.e., $\mathbf{C}=\mathbf{I}_{n_x}$) where $\pi(\cdot)$ is an $m$-layer feedforward NN.
Denote the closed-loop system \cref{eqn:ltv_dynamics} and control policy $\pi$ as 
\begin{equation}
    \mathbf{x}_{t+1} = f(\mathbf{x}_{t}; \pi). \label{eqn:closed_loop_dynamics}
\end{equation}

\subsection{Control Policy Neural Network Structure}

% For a feedforward NN with $L$ hidden layers (and two additional input and output layers), the number of neurons in each layer is $n_l\in[L+1]$, where $[i]$ denotes the set $\{0,1,\ldots,i\}$.
% We introduce the $l$-th layer's weight matrix $\mathbf{W}^{(l)}\in\R^{n_{l+1}\times n_{l}}$, bias vector $\mathbf{b}^{(l)}\in\R^{n_{l+1}}$, and coordinate-wise activation function $\sigma^{(l)}: \R^{n_{l+1}} \to \R^{n_{l+1}}$, which can include tanh, sigmoid, ReLU (i.e., $\sigma(\mathbf{z})=\mathrm{max}(0,\mathbf{z})$), and many others.
% For input $\x\in\R^{n_0}$, the NN output $\pi(\x)$ is,
% \begin{align}
% \begin{split}
%     \x^{(0)} &= \x \\
%     \z^{(l)} &= \mathbf{W}^{(l)} \x^{(l)}+\mathbf{b}^{(l)}, \forall l\in[L] \\
%     \x^{(l+1)} &= \sigma^{(l)}(\z^{(l)}), \forall l\in[L-1] \\
%     \pi(\x) &= \z^{(L)}.
% \end{split}
% \end{align}

Consider a feedforward NN with $L$ hidden layers and two additional layers for input and output.
We denote the number of neurons in each layer as $n_l\ \forall l \in [L+1]$ where  where $[i]$ denotes the set $\{0,1,\ldots,i\}$.
The $l$-th layer has weight matrix $\mathbf{W}^{l}\in\R^{n_{l+1}\times n_{l}}$, bias vector $\mathbf{b}^{l}\in\R^{n_{l+1}}$, and activation function $\sigma^{l}: \R^{n_{l+1}} \to \R^{n_{l+1}}$, where $\sigma^{l}$ can be any option handled by CROWN~\cite{zhang2018efficient}, e.g., sigmoid, tanh, ReLU, etc. For an input $\x\in\R^{n_0}$, the NN output $\pi(\x)$ is computed as
\begin{align}
\begin{split}
    \x^{0} &= \x \\
    \z^{l} &= \mathbf{W}^{l} \x^{l}+\mathbf{b}^{l}, \forall l\in[L] \\
    \x^{l+1} &= \sigma^{l}(\z^{l}), \forall l\in[L-1] \\
    \pi(\x) &= \z^{L}.
\end{split}
\end{align}

\subsection{Neural Network Robustness Verification}

% A key step in efficiently conducting reachable set analysis of an NFL~\cref{eqn:closed_loop_dynamics} is to relax the nonlinearities introduced by the NN's activation functions. By converting the nonlinearities in the activation function into an affine upper and lower bound, where each bound holds for the known range of inputs to the NN, we can obtain a simplified relationship between the NN's input and output. 

% We represent the range of inputs to the activation functions with the $\epsilon$-ball (also called the $\ell_p$-ball).
% Denote the $\epsilon$-ball under the $\ell_p$ norm, centered at $\xnom$, with scalar radius, $\epsilon$,
% \begin{align}
%     \bpxnomscalar &= \{\mathbf{x}\ \lvert\ \lvert\lvert \mathbf{x} - \xnom \rvert \rvert_p \leq \epsilon \}.
% \end{align}
% The $\epsilon$-ball is extended to the case of vector $\bm{\epsilon}\in\R^n_{\geq 0}$ (i.e., $\bm{\epsilon}$-ball), defined as
% \begin{align}
%     \bpxnom &= \{\mathbf{x}\ \lvert\ \lim_{\bm{\epsilon}' \to \bm{\epsilon}^+} \lvert\lvert (\mathbf{x} - \xnom) \oslash \bm{\epsilon}' \rvert\rvert_p \leq 1\},
% \end{align}
% where $\oslash$ denotes element-wise division.

To avoid the computational cost associated with calculating exact BP sets, we relax the NN's activation functions to obtain affine bounds on the NN outputs for a known set of inputs.
The range of inputs are represented using the $\ell_p$-ball 
\begin{align}
    \bpxnom &\triangleq \{\mathbf{x}\ \lvert\ \lim_{\bm{\epsilon}' \to \bm{\epsilon}^+} \lvert\lvert (\mathbf{x} - \xnom) \oslash \bm{\epsilon}' \rvert\rvert_p \leq 1\},
\end{align}
where $\xnom \in \R^n$ is the center of the ball, $\bm{\epsilon}\in\R^n_{\geq 0}$ is a vector whose elements are the radii for the corresponding elements of $\mathbf{x}$, and $\oslash$ denotes element-wise division.



% Given an $m$-layer neural network function $f : \R^{n_0} \rightarrow \R^{n_m}$, there exists two explicit functions $f^L_j : \R^{n_0} \rightarrow \R$ and $f^U_j :\R^{n_0} \rightarrow \R$ such that $\forall j \in [n_m], \; \forall \x \in \Ball$, the inequality $\, f_{j}^{L}(\x) \leq f_{j}(\x) \leq f_{j}^{U}(\x)$ holds true, where
\begin{theorem}[\!\!\cite{zhang2018efficient}, Convex Relaxation of NN]\label{thm:crown_particular_x}
Given an $m$-layer neural network control policy $\pi:\R^{n_x}\to\R^{n_u}$, there exist two explicit functions $\pi_j^L: \R^{n_x}\to\R^{n_u}$ and $\pi_j^U: \R^{n_x}\to\R^{n_u}$ such that $\forall j\in [n_m], \forall \mathbf{x}\in\bpxnom$, the inequality $\pi_j^L(\mathbf{x})\leq \pi_j(\mathbf{x})\leq \pi_j^U(\mathbf{x})$ holds true, where
\begin{equation}
\label{eq:f_j_UL}
    \pi_{j}^{U}(\x) = \CROWNAu_{j,:} \x + \CROWNbu_j, \quad
    \pi_{j}^{L}(\x) = \CROWNAl_{j,:} \x + \CROWNbl_j,
    % \pi_{j}^{U}(\y) &= \Au{(0)}_{j,:} \y + \sum_{k=1}^{m}\Au{(k)}_{j,:}(\bias{(k)}+\upbias{(k)}_{:,j}) \\
    % \pi_{j}^{L}(\y) &= \Al{(0)}_{j,:} \y + \sum_{k=1}^{m}\Al{(k)}_{j,:}(\bias{(k)}+\lwbias{(k)}_{:,j}),
\end{equation}
where $\CROWNAu, \CROWNAl \in \R^{n_u \times n_x}$ and $\CROWNbu, \CROWNbl \in \R^{n_u}$ are defined recursively using NN weights, biases, and activations (e.g., ReLU, sigmoid, tanh), as detailed in~\cite{zhang2018efficient}.
\end{theorem}

% \subsection{Backward Reachability Analysis}\label{sec:backward_reachability}

% In this section, we discuss the problem of \textit{backward} reachability: given a target set $\mathcal{X}_T$, from which states will the system end up in the target set?


\subsection{Backreachable \& Backprojection Sets}

\begin{figure}[t]
\begin{tikzpicture}

    \draw [red, ultra thick] (2,1) rectangle (4,2) node[above] {$\mathcal{X}_{T}$};
    
    \draw [fill=black!20!green!60!white]  plot[smooth, tension=.7] coordinates {(-3,2.5) (-3.5,2.2) (-4,1.5) (-3.5,0) (-3.5,-1.8) (-2.5,-1.9) (-0.3,-2) (0.,-1) (-0.3,0) (-1,1.5) (-2.5,2.5) (-3,2.5)} node[above] {$\mathcal{R}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (a) at (-2,2) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (b) at (3,1.5) {};
    \draw [->,blue, ultra thick] (a.east) to [out=0,in=150] (b.north);
    \node[black] (RTset) at (-0,2.4) {$\exists \mathbf{u} \in \mathcal{U}$};

    \draw [fill=black!10!white]  plot[smooth, tension=.7] coordinates {(-3.0,1.4) (-1.5,1.3) (-0.2,-1.0) (-1.1,-1.8) (-3.2,-1.2) (-3.0,1.4)} node[above] {$\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c) at (-0.6,-1.5) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d) at (3.8,1.1) {};
    \draw [->,blue, ultra thick] (c.east) to [out=0,in=300] (d.south);
    \node[black] (PTbarset) at (2.1, -1.8) {$\exists \mathbf{u} \in [\pi^L(\mathbf{x}_{-1}), \pi^U(\mathbf{x}_{-1})]$};

    \draw [fill=black!40!white]  plot[smooth, tension=.7] coordinates {(-2.3,0.8) (-1.5,0.7) (-0.5,-0.8) (-1.4,-1.6) (-2.8,-0.8) (-2.3,0.8)} node[above] {$\mathcal{P}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (e) at (-2.2,0.6) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (f) at (2.3,1.5) {};
    \draw [->,blue, ultra thick] (e.east) to [out=0,in=180] (f.west);
    \node[black] (PTset) at (0.3, 1.6) {$\mathbf{u} = \pi(\mathbf{x}_{-1})$};

    \draw [fill=black!20!white]  plot[smooth, tension=.7] coordinates {(-1.84,-0.1) (-1.5,-0.6) (-0.6,-0.8) (-1.1,-1.4) (-2.8,-0.8) (-1.84,-0.1)} node[above] {$\ubar{\mathcal{P}}_{-1}(\mathcal{X}_T)$};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (c) at (-1.9,-.25) {};
    \node[circle,fill=black,inner sep=0pt,minimum size=3pt] (d) at (2.5,1.1) {};
    \draw [->,blue, ultra thick] (c.east) to [out=10,in=170] (d.west);
    \node[black] (PTbarset) at (1.65, 0.15) {$\forall \mathbf{u} \in [\pi^L(\mathbf{x}_{-1}), \pi^U(\mathbf{x}_{-1})]$};

\end{tikzpicture}
\caption{
Backreachable, backprojection, and target sets.
Given a target set, $\mathcal{X}_T$, the backreachable set $\mathcal{R}_{-1}(\mathcal{X}_T)$ contains all states for which \textit{some} control exists to move the system to $\mathcal{X}_T$ in one timestep.
BP set $\mathcal{P}_{-1}(\mathcal{X}_T)$ contains all states for which the NN controller leads the system to $\mathcal{X}_T$.
BP under-approximation $\protect\ubar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ and over-approximation $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ contain states for which \textit{all} and \textit{some}, respectively, controls that the relaxed NN could apply lead the system to $\mathcal{X}_T$.
}
\label{fig:backreachable}
\vspace*{-0.12in}
\end{figure}

% \cref{fig:backreachable} illustrates the important concepts for this analysis.
% Four different sets (left) contain states that lead to the target set $\mathcal{X}_T$ (right) under different requirements on the control inputs, as defined below.
% The nomenclature of these sets is inspired by~\cite{lavalle2006planning} with a slight modification of the definitions.
% %
% The first of these sets is the \textit{backreachable set}, 
% \begin{align}
% % \begin{split}
%     \mathcal{R}_{t-1}(\mathcal{X}_T) &= \{ \mathbf{x}\ \lvert\ \exists\mathbf{u} \in \mathcal{U} \mathrm{\ s.t.\ } \label{eqn:backreachable_sets} \\
%      &\mathbf{A}\mathbf{x} + \mathbf{B}\mathbf{u} + \mathbf{c} \in \mathcal{R}_t(\mathcal{X}_T) \}\ \forall t \leq 0  \nonumber \\
%     \mathcal{R}_0(\mathcal{X}_T)&=\mathcal{X}_T, \nonumber
% % \end{split}
% \end{align}
% which consists of states $\mathbf{x}_t$ for which some admissible (i.e., within the control limits) control trajectory, $\mathbf{u}_{t:T}$, takes the system to $\mathcal{X}_T$.
% % To simplify the notation, we assume no noise (i.e., $\ubar{\bm{\omega}}_t = \bar{\bm{\omega}}_t = \ubar{\bm{\nu}}_t = \bar{\bm{\nu}}_t = \mathbf{0}$) and perfect observations, $\mathbf{C}^T_t = \mathbf{I} \Rightarrow \mathbf{y}_t = \mathbf{x}_t$ in this section.
% The backreachable set is a good starting point for backward reachable set analysis because its definition only uses the fact that $\mathbf{u}\in\mathcal{U}$, rather than $\pi$.

% Given a NN control policy, we can be more precise about the closed-loop system's safety properties.
% In particular, for the closed-loop system $f(\mathbf{x}_{t}; \pi)$ from~\cref{eqn:closed_loop_dynamics}, we denote $\mathcal{P}_{-t}(\mathcal{X}_T)$ the backprojection set, which contains all states that the NN will drive to a given target set $\mathcal{X}_T\subseteq\R^{n_x}$ in exactly $t$ timesteps, as defined by the recursion
% \begin{align}
% % \begin{split}
%     \mathcal{P}_{t-1}(\mathcal{X}_T) &= \{ \mathbf{x}\ \lvert\ \mathbf{A}\mathbf{x} + \mathbf{B}\pi(\mathbf{x}) + \mathbf{c} \in \mathcal{P}_t(\mathcal{X}_T) \} \label{eqn:backprojection_sets} \nonumber \\
%     & \quad\quad \forall t \leq 0 \nonumber \\
%     \mathcal{P}_0(\mathcal{X}_T)&=\mathcal{X}_T.
% % \end{split}
% \end{align}
% The final two sets shown in~\cref{fig:backreachable} are $\bar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ and $\ubar{\mathcal{P}}_{-1}(\mathcal{X}_T)$ which define over- and under-approximations, respectively, of $\mathcal{P}_{-1}(\mathcal{X}_T)$.
% Comparison of the motivation behind over- and under-approximation strategies is given in the next section.

The distinction between sets used in this work is shown in \cref{fig:backreachable}.
Given a target set $\mathcal{X}_T$ (right), each of the four sets on the left contain states that will reach $\mathcal{X}_T$ under different conditions on the control input $\mathbf{u}$, described below.

First, the one-step backreachable set
% \begin{align}
%     \mathcal{R}_{-1}(\mathcal{X}_T) &= \{ \mathbf{x}\ \lvert\ \exists\mathbf{u} \in \mathcal{U} \mathrm{\ s.t.\ } \label{eqn:backreachable_sets} \\ \nonumber
%      &\mathbf{A}\mathbf{x} + \mathbf{B}\mathbf{u} + \mathbf{c} \in \mathcal{X}_T \}\
% \end{align}
\begin{equation}
    \mathcal{R}_{-1}(\mathcal{X}_T) \triangleq \{ \mathbf{x}\ \lvert\ \exists\mathbf{u} \in \mathcal{U} \mathrm{\ s.t.\ } \label{eqn:backreachable_sets}
     \mathbf{A}\mathbf{x} + \mathbf{B}\mathbf{u} + \mathbf{c} \in \mathcal{X}_T \},
\end{equation}
contains the set of all states that transition to $\mathcal{X}_T$ in one timestep given some $\mathbf{u}\in \mathcal{U}$.
The importance of the backreachable set (or at least an over-approximation to the backreachable set, as will be seen later) is that it only depends on the control limits $\mathcal{U}$ and not the NN control policy $\pi$.
Thus, while $\mathcal{R}_{-1}(\mathcal{X}_T)$ is itself a very conservative over-approximation of the true set of states that will reach $\mathcal{X}_T$ under $\pi$, it provides a region over which we can relax the NN with forward NN analysis tools, thereby avoiding issues with NN invertibility.

Next, we define the one-step true BP set as
\begin{equation}
    \mathcal{P}_{-1}(\mathcal{X}_T) \triangleq \{ \mathbf{x}\ \lvert\ \mathbf{A}\mathbf{x} + \mathbf{B}\pi(\mathbf{x}) + \mathbf{c} \in \mathcal{X}_T \}, \label{eqn:backprojection_sets}
\end{equation}
which denotes the set of all states that will reach $\mathcal{X}_T$ in one timestep given the input from $\pi$.
As previously noted, calculating $\mathcal{P}_{-1}(\mathcal{X}_T)$ exactly is computationally intractable, which motivates the development of approximation techniques.
Thus, the final two sets shown in~\cref{fig:backreachable} are the BP set over-approximation 
\begin{align}
    \bar{\mathcal{P}}_{-1}(\mathcal{X}_T) &\triangleq \{ \mathbf{x}\ \lvert\ \exists\mathbf{u} \in [\pi^L(\x), \pi^U(\x)] \mathrm{\ s.t.\ } \label{eqn:backprojection_set_over} \\ \nonumber
     &\mathbf{A}\mathbf{x} + \mathbf{B}\mathbf{u} + \mathbf{c} \in \mathcal{X}_T \},\
\end{align}
and BP set under-approximation
\begin{align}
    \ubar{\mathcal{P}}_{-1}(\mathcal{X}_T) &\triangleq \{ \mathbf{x}\ \lvert\ \forall\mathbf{u} \in [\pi^L(\x), \pi^U(\x)] \mathrm{\ s.t.\ } \label{eqn:backprojection_set_under} \\ \nonumber
     &\mathbf{A}\mathbf{x} + \mathbf{B}\mathbf{u} + \mathbf{c} \in \mathcal{X}_T \}.\
\end{align}
Comparison of the motivation behind over- and under-approximation strategies is given in the next section.

\subsection{Backprojection Set: Over- vs. Under-Approximations}

The need to approximate the BP set naturally leads to the question of whether we should compute over- or under-approximations.
Both types of BP set approximations have relevant physical meaning and are valuable for different reasons.
An under-approximation is useful if the target set is a goal set, because we aim to find a set of states at the previous timestep that will \textit{certainly} drive the system into the goal set.
% In other words, we do not want the system to miss the goal because the NN relaxation is too loose.
This leads to a ``for all'' condition on the relaxed NN (i.e., $\forall \mathbf{u} \in [\pi^L(\x), \pi^U(\x)]$) in \cref{eqn:backprojection_set_under}. Conversely, an over-approximation is useful if the target set is an obstacle/avoid set, because we aim to find all states at the previous timestep for which $\pi$ \textit{could} drive the system into the avoid set.
% In other words, we do not want the system to collide with the obstacle because the NN relaxation is too loose.
This leads to an ``exists'' condition on the relaxed NN (i.e., $\exists \mathbf{u} \in [\pi^L(\x), \pi^U(\x)]$) in \cref{eqn:backprojection_set_over}. Note that in this work we use ``over-approximation'' and ``outer-bound'' interchangeably.

Ref.~\cite{everett2021reachability} introduced a closed-form equation capable of one-step under-approximations of BP sets.
Unfortunately, this closed form equation hinged on the ``for all'' condition and thus cannot be used to generate BP set over-approximations, necessitating a different approach. % is not apparent, necessitating a different approach.
% In this work, we provide two algorithms for computing multi-step over-approximations of the BP sets that can be used to verify that the system will not enter an unsafe region of the state space over a given time horizon.
\fi


